Communicative Visualizations as a Learning Problem

Significant research has provided robust task and evaluation languages for the analysis of exploratory visualizations. Unfortunately, these taxonomies fail when applied to communicative visualizations. Instead, designers often resort to evaluating communicative visualizations from the cognitive efficiency perspective: "can the recipient accurately decode my message/insight?" However, designers are unlikely to be satisfied if the message went 'in one ear and out the other.' The consequence of this inconsistency is that it is difficult to design or select between competing options in a principled way. The problem we address is the fundamental mismatch between how designers want to describe their intent, and the language they have. We argue that visualization designers can address this limitation through a learning lens: that the recipient is a student and the designer a teacher. By using learning objectives, designers can better define, assess, and compare communicative visualizations. We illustrate how the learning-based approach provides a framework for understanding a wide array of communicative goals. To understand how the framework can be applied (and its limitations), we surveyed and interviewed members of the Data Visualization Society using their own visualizations as a probe. Through this study we identified the broad range of objectives in communicative visualizations and the prevalence of certain objective types.

==> 05_Qual.tex <==




==> 99_scratch.tex <==
Insights are a familiar idea to those producing communicative visualizations~\cite{stasko2014value}. `Bigger than insights' are knowledge elements that go beyond simple facts to include concepts, theories, groupings, processes, etc. It is an easier starting point for a student to identify visualization techniques to focus on insights (e.g., through annotations, captions, associated text, and visual highlights of graphical elements). `Bigger' creates a useful challenge. 




Communicative visualizations are prevalent, increasingly sophisticated (e.g., highly interactive visualizations on news sites), and often have a significant audience and impact. Because of this growing impact, it is vital to ensure that the goals of the designer are articulated. As critically, the designer should understand the effect, both desired and undesired, on the audience. While other areas in HCI (e.g., UX design) and visual analytics have crafted ``languages'' for modeling end-users, designers of communicative visualization rely on generic guidelines, instinct, and very few theoretical or practical tools. Because it is hard for the designer to explicitly articulate what the designer wants to achieve--which insights they want the audience to take away, and what `take away' actually means--it is difficult or impossible to execute good evaluations. Even in the process of design, a workflow that encourages clear descriptions of these goals benefits the designer by forcing clarity about their objectives \textit{in the design phase}. 


There are both historic and pragmatic reasons why we lack a detailed task language for communicative visualizations. However, there are a number of trends that make this gap more pronounced and the need more apparent. First, we have moved from very simple statistical charts and diagrams (a bar chart, a pie plot, etc.) that were well captioned and annotated. Modern communicative designs can now offer radically different designs featuring complex encoding, interactivity, and structure. 

Narrative techniques offer one way to manage this complexity~\cite{Segel2010, rhetoric,hullman2013b}. Unfortunately, narrative techniques at best provide strategies and do not describe testable design goals. LOs address this by providing the designer with a flexible (but structured) way to describe their \textit{intent}. An objective can be very narrow (e.g., ``the reader be able to identify the maximum rain-fall value'') or broad (e.g., ``the reader will be able to determine the networked flow of capital between any pair of international banks''). This flexibility ensures that both simple and complex visualizations can be modeled. As critically, good LOs lead to good assessments. An articulation of what a reader \textit{will be able to do}, can be naturally transformed into an assessment if, after seeing the visualization, \textit{they can}. For example, for the `rain' objective above we can ask: ``Which state has the highest rainfall? (A) Hawaii, (B) Washington, (C) Alabama.'' For the bank case, we might ask ``Which of the following is the amount of cash transferred between Novobank and Bankotech? (A) 5.3M, (B) 4.2M, (C) 7M.'' These questions can be generated semi-automatically and their difficulty manipulated.

The second problem for communicative visualizations is they are often `one-offs.' Generic task-languages (e.g., identifying outliers in a social network), or even domain-specific workflows (e.g., identifying genes) are not specific enough for many communicative visualization problems. For example, take the \textit{New York Times'} interactive visualization for communicating the network structure of soccer player clubs around the World Cup (see Figure~\ref{fig:soccer}). When they built this visualization, the \textit{Times} designers were not building a system to support broad social network analysis, but rather picking specific, narrow, data-specific insights, about the connection of player and clubs, to provide to the reader. Learning objectives are formulated as: ``The reader will \textul{verb} \textul{noun}.'' The verbs (the type of cognitive process a student should display) and nouns (the knowledge a student should attain) are well-suited for high-specific communicative visualizations. Those constructing learning objectives are strongly dissuaded from using generic language (e.g., ``The reader will be able to \textit{understand}...'') and focusing on specific forms (e.g., explain, describe, recall, etc.). 

A final difference for communicative visualization is the push-versus-pull problem. Traditionally, visual \textit{analytics} is a \textit{pull}-type problem. The goals are motivated by \textit{the user}. It is possible to model what the user wants, or may want, and evaluate based on this model. Conversely, communicative visualization is a \textit{push}-type problem. The goals are \textit{the designer's}, and may only partially (or not at all) take into account the wants and tasks of the user (i.e., reader). Because of this, current methods for describing the intent (e.g., task models) and evaluation are not readily carried over to communicative visualization. Learning objectives, conversely, target the goals of the instructor (i.e., designer) and a key function of assessment techniques is for the instructor to judge the efficacy of their teaching. Or in our case, for the designer to judge the efficacy of their visualization.  We note that while high-level goals such as `engagement' are supported within the LO language, LOs encourage the designer to answer the question `engagement to what end?' Our work is motivated by using engagement to aid learning~\cite{CHEN20101222}. Our goal is to explicitly separate measuring learning outcomes with business metrics. Engagement or `retention' as a business goal (e.g., ad revenue) can be measured by other mechanisms and integrated into decisions on which visualizations to produce~\cite{doi:10.1177/1094670510375599, doi:10.1177/1094670510375603}. 


\underline{Background:} While a broad test catalog (\textbf{T-Structure}) is useful, designers need to be able to transform LOs into usable test items. This transformation requires both the construction of the test item and the answer key. The process varies for CR and MC formats. CR formats, for example,  requires constructing a rubric~\cite{haladyna2012developing}. 

``Studies in CTV are often intended to quantify a tool’s
quality through metrics such as learning rate, information
1. This was an earlier iteration of insight-based evaluation, different
from the longitudinal study mentioned above
JOURNAL SUBMISSION 8
retention and accuracy, or qualitative metrics such as interaction
patterns of the way people absorb information
or approach the tool. Questions thus pertain to the quality
with which information is acquired and the modalities with
which people interact with the visualizations. Examples are:

~\cite{krathwohl1956taxonomy}
1.0 Receiving (attending)
1.1 awareness
1.2 Willingness to receive
1.3 Controlled or selection attention
2.0 Responding
2.1 Acquiescence in responding
2.2 Willingness to respond
2.3 Satisfaction in response
3.0 Valuing
3.1 Acceptance of a value
3.2 Preference for a value
3.3 Commitment (conviction)
4.0 Organization
4.1 Conceptionalizion of a value
4.2 Organization of a value system
5.0 Characterization by a value or value complex
5.1 Generalized set
5.2 Characterization

1.0 Receiving 1.1 Awareness (create a pleasant environment) –
senses, sees, listens, perceives, is aware 1.2 Willingness (lesson initiation – “motivating, gaining, and keeping [the] student’s attention”
– offers, watches, listens, tolerates, is willing, chooses, eagerness 1.3
Attentiveness – attends given distractions – observes, concentrates,
attends, is interested, is focused 2.0 Responding 2.1 Acquiescing –
disposition to accept ideas/actions as suggested by others as worthwhile – acquiesces, accepts, agrees, allows 2.2 Complying – disposition to act with little or no prompting – agrees, complies, observes,
follows, obeys, conforms, cooperates, volunteers 2.3 Assessing – disposition to appraise one’s feelings about what was received and one’s
response to it – likes/dislikes, wants to/does not want to, enjoys, is interested/uninterested, felt activity was easy/hard, was satisfied/unsatisfied,
is sure/unsure, is ambivalent 3.0 Valuing 3.1 Accepting – disposition
to endorse a basic value – accepts, agrees, endorses, selects, rejects,
opposes 3.2 Preferring – disposition to discriminate among alternative
values – favors, selects, prefers, supports, chooses, compares, discriminates 3.3 Confirming – disposition to verify the worth of a value
through rationalization or experience – verifies, concludes, rationalizes,
tests, justifies, supports, validates, confirms, judges, is disposed to
should/should not, would/would not 4.0 Believing 4.1 Trusting – disposition to have confidence in and rely on a value as a guiding principle
– trusts, views, relies, values, believes 4.2 Committing – disposition
to internalize and adhere to a value as a guiding principle – supports,
participates, persists, practices, joins, adheres, complies 5.0 Behaving
5.1 Demonstrating – disposition to act in accord with a value of belief –
does, acts, performs, behaves, demonstrates, practices, serves, uses 5.2
Modifying – a disposition to adjust or refine one’s behaviors in accord
with values and beliefs – adjusts, modifies, refines, corrects, alters
 
 
 But may not be easy to induce attitude change~\cite{Kong:2018:FST:3173574.3174012}
 
 \subsection{incentives}
The issue of incentives -- are ar enot incentivizing an answer. The student isn't being evaluated, we are evaluating the program. The issue of not answering the question (specfically the affective type) may be a non-issue: ``A considerable part of the hesitation in the use of affective measures for grading purposes stems from the inadequacy of the appraisal techniques and the ease with which a student may exploit his ability to detect the responses which will be rewarded and the responses which will be penalized.''

Data art -- subset of communicative visualization where we remove cognitive objectives and focus on affective objectives

If we want to politicize data we can do it by specifying a specific set of affective objectives

having a netural affect (the anti-LO) can be explicit value and learning objective 




Good examples: Obamacare network/vis, global warming animation, vaccination example


Fink~\cite{fink2013creating}--complaint of the limitation of bloom to cognitive, seeks to re-integrate affective (drawn in circle/pie)---all integrate to create \textit{signficant learning}. Foundational knowledge (understanding and remembering, information/ideas), Application (skills, thinking--critical, creative, and practical, managing projects), integration (connecting, ideas, peoples, realms of life), Human dimension (learning about oneself, others), Caring (Developing new: feelings, interest, values), Learning how to learn (Becoming a better student, inquiring about a subject, self-directing learners).


Based on our findings in determining objectives suitable for communicative visualization (\textbf{L-Objectives}) our second goal is to identify suitable forms of assessment. By leveraging the existing literature and experimentation, we will identify the strengths and weaknesses of the formats in relation to communicative visualization LOs. We will produce a broad catalog of possible assessments driven by the \textbf{L-Objectives} data. We will then group these by `equivalence,' and deploy variants through Amazon's mTurk to identify possible strengths and weaknesses (e.g., are some forms harder to understand than others? do some populations do better with one form over another?).




The process of producing LOs has a number of benefits~\cite{anderson2001taxonomy, gronlund2008gronlund}. First, it informs students of the goals of the class (less critical in our case). Second, it supports the construction of assessments. Third, it ensures that the instructor creates an effective curriculum. 


However, a promising structure makes use of `item shell' and `item modelling' approaches for building multiple choice questions~\cite{doi:10.1080/095006999290714, haladyna2012developing}. With item shells, the designer applies a set of concrete steps to transform questions into templates and from those produce new test items. For example, given a patient dataset including age, accident type, and `presentation'  a validated test question might be: ``For a six-year-old child, how often would we expect to see a broken arm from a car accident?'' The item shell method proceeds by (1) identifying `content' items (here it would be `six-year-old,' `broken arm,' and `accident'); (2) identifying variations (e.g., the age `slot' could be 0-99, the 'presentation' type might be broken arm, cuts, bruising, etc.); (3) selecting new age/incident type/presentation triplets and inserts them into the template.  For this research question, we will produce a method for generating test items. We will compare techniques that the original LOs, insight examples, and example questions. We will also identify which data and visualization properties (e.g., visualization or data types) may indicate that specific techniques are better. For this question we will utilize mTurk workers and students with education training.

Constructed Response (CR) versus Multiple Choice (MC)

Observation: if we accept that LOs are good ways to describe what we want to achieve, this opens up a wide range of assessment tools






Haladyna - focus on knowledge, skills, and abilities

Haladyna - Cronbach -- validation: formulation (define the construct, hypothesis), explication (construction of measure), and validation (check if hypothesis holds)


Future work: what is the right test format. Validity arguments by Holdanaya: prediction (does test predict something), content equivalence (does it matter if we use CR or MC), proximity to criterion (fidelity, proximity), bias (e.g., gender/format), cognitive demand validity (MC items that elicit complex behaviors are hard to design), instrumentality


Holdonoya - knowledge and cognitive processes .  Cognitive process :

Knowledge -- Recalling/understanding -- split into fact, concept, principle, procedure. Holdonya example ``draw conclusions from graphed data'' relates to principle knowledge. Recall -- repeat as stated, Understand -- paraphrase

Skill -- Application of process

Ability -- complex structure that includes a large domain of knowledge and skills


Application of information in making a decision (skill assessment) -- LO. 

Halda - high inference versus low inference outcomes (ones where we can have concrete observation) as key factor in picking item format

\subsection{Workflows}
**Note: contrast to Miriah's workflow. Does it fit in there?

Look at data notebook stuff... can we make the argument that this is worflow compatible? It's not a drop-in replacement... it's a new and hard step but one that doesn't break process.

Does it fit to educational theory and instructional design workflows? Maybe, but those tend to be higher level (this would be a micro-decision in the broader educational framework)~\cite{seels1990exercises}

Backward design [understanding by design stuff]

UX design workflows?

Embedding of visualization in context... can't separate the context from the vis. They are integral. Example: same vis in different context (the text in, the text around, the reader, the venue).''

How do we know we have the right level of detail? Pick one that is reasonable to expect as an outcome of the change *due* to the visualization. If the vis is unlikely to allow us to meet the objective, it's a bad objective (not a bad vis).


LOs are the right thing for us.

\subsection{Difficulty and training}

**Note: anything to say about difficulty in learning how to make learning objectives? Part of the driver for having so many varieties.. instructors find it hard

\subsubsection{Goals, Objectives, and Outcomes}
Those familiar with the education literature may appreciate the difference between goals, objectives, and outcomes (but may still struggle to define them when called upon). The interesting question is more about the level of granularity that would support our process.~\cite{harden,prideaux}

\subsection{Considering your audience}
Mediator: visual literacy
Mediator: ...






Munzner's multilevel stuff is focused on user-centered tasks. Good breakdown into steps and the consume part is (present, enjoy, produce) is really about what the user wants to do. Does not really help us construct objectives at the right granularity or assess success.  Focus on features rather than goals.  This vis will allow/support [X]... (outcomes of engineering effort), 
Knowledge dimension missing. Critical piece.

\subsection{Bad objective}
redundant, untestable~\cite{waller2001writing}
able to 
shows interest in
appreciation for 
knows
awareness of 
has knowledge of
capable of 
learns
comprehend 
memorizes
conscious of 
understands
familiar with 
will be able to 

Bertin -- query system. three levels of reading: elementary, intermediate, and overall. Focus on agency of reader. ``...CHOOSE PREFERRED QUESTIONS and construct the graphic so they can be answered in a single instant of perception.''~\cite{bertin}

Recording, communicating, processing

. The Philip's curve question above is called a multiple true-false format. 

For example we could ask: ``In which of the following periods did correlation vanish between unemployment and inflation? (a) 1980-1990, (b) 1991-2000, or (c) 2001-2010'' (multiple choice); and ``In which of the following periods did correlation vanish between unemployment and inflation (label each with a true-false): (a) 1980-1990? (b) 1991-2000? (c) 2001-2010?'' (multiple true-false). 


Additionally, with strategic use of test items, participants may be able to find not just \textit{which} visualization is better, but \textit{why} by identifying which of competing perception  theories are at work~\cite{doi:10.1080/01621459.1987.10478448, TOPS:TOPS1066,pinker1990theory,Hegarty2004}.

However, engagement is somewhat vague 

Pays to be honest by what we mean by engagement. Is Engagement purely a \$ driver (show more ads)? in which case it's not really about the user.

Is engagement an instructional strategy to achieve better learning outcomes? In which case the objective is something else... getting you to engage buys you the attention to achieve the objective.

Is engagement actually a broader value about wanting the reader to attend to a set of facts and literature? In this case we can call it what it is and use one of the affective learning objective terms.

Pays to be honest here. Could be a mix of these things.

At first we pick up only one or few aspects of the task (unistructural), then several aspects but they are unrelated (multistructural), then we learn how to integrate them into a whole (relational), and finally, we are able to generalised that whole to as yet untaught applications (extended abstract). The diagram lists verbs typical of each such level.

SOLO - Biggs Structure of Observed Learning Outcomes (SOLO), attractive because it uses a cool diagram.  Pre-Structural (brain dump), Uni-structural (influence of nature on X, or simply describe words), Multi-structural, Relational, Extended Abstract.
No Idea - equivalent to the prestructural level.
One Idea - equivalent to the unistructural level
Many Ideas - equivalent to the multistructural level
Relate - equivalent to the relational level
Extend - equivalent to the extended abstract


Prestructural (no idea-possibly wrong inferences about the data), Unistructural (simple extraction of few items from visualization... value of X is Y, likely the annotated one), Multistructural (understanding of pulling the values of each bar, possibly rebuilding the datset), Relational (understanding the significance of the visualization as a whole), extended abstract (...)

Worksheet -- stage 1: Desired reults (defined: established goals, define understandings and essential questions, describe objectives... students will know, students will be able to...), staeg 2: assessment evidence (performance tasks, other evidence), stage 3--learning plan (WHERETO)


WHERETO eleemnts: W -- WHERE and WHY and unit is heading, H - Hook and hold attention, E - Equip with necessary stuff, R -- provide oppotunities to rethink, reflect, and revise, E -- build oppotunities to evaluate progress, T -- be tailored, O -- be organized

. key idea: backward design. Explicitly pull out \textit{Enduring Understandings}--things that transfer. 



Depth of Knowledge~\cite{webb2002depth}
     Recall (or Recognition)
      Basic Application
      Strategic Thinking
      Extended Thinking
      
      
      
Cairo: ``The first and main goal of any graphic and visualization is to be a tool for your eyes and brain to perceive what lies beyond their natural reach.''

But why limit ourselves to pedagogic images... all communication is pedagogic (note: MEMORIZABLE not MEMORABLE)

passive analyst -- Bertin: ``What matters less is the number of correspondences retained, provided that these are esssential ones. The image can be NONCOMPREHENSIVE. With this function, the graphic is a `MESSAGE.' Its efficiency increases as the number of images (superimposed or seperate) and their complexiy diminish as reading approaches the OVERALL LEVEL.''

``How can the comprehensive information be reduced, the smallest number of simplified images determined, so that the information becomes communicable and memorizable, \textit{without being falsified or destroyed}? How can this choice be justified? Is a choice always necessary?''

(the incentive issue), but we can still have andragogy (adult learning). learning objectives are no less meaningful here, we just need to mediate them with 



Seperation between graphic as a storage mechanism that REPLACES human memory and form which becomes INSCRIBED in human memorty


In many instances, visualization engineering is a form of `wicked design.' Like instruction, the designer must prioritize which knowledge is most important for a student to take away.  In the design of visual analytics systems this process is often manifested as an iterative design process~\cite{Sedlmair:2012:DSM:2720013.2720398} where feedback from the end-user drives design.


In addition to 
What people come in with... knowledge, background, predisposition.  Sometimes called input (but broadly the context).  Affect: morals, customs, theologies, philosophies, laws, etc.

We propose to leverage a subset of Bloom's taxonomy~\cite{bloom1956taxonomy}, and specifically the revised version~\cite{anderson2001taxonomy}.  Though there are other related taxonomies as the DIKW knowledge hierarchy~\cite{dikw,zins07} or the six facets of  understanding~\cite{wiggins2005understanding}, the revised Bloom's taxonomy is well studied and can be readily adapted to assessment.  

These `nouns' range from factual to meta-cognitive. At the intersection of the dimensions are specific verbs to describe the objective.  For example, the intersection of factual (knowledge) and remember (cognitive) includes `list,' as in: ``The reader will be able to list the rainfall levels in the western states.'' The assumption is that after exposure to the educational materials--in our case the visualization--the reader will be able to achieve this objective.  

``The result was a sophisticated way to watch the election unfold, giving readers a much better sense of how close the race really looked.'' -- nytimes

Questionable hierarchy. Not focused on behaviors. Objections to whether it was systematic enough. Objections to whether it was hierarchical enough but simultaneously that in being a hierarchy that teachers would focus on the `peak.' Often drawn as pyramid but that's not really the intent


Create a shift from \textit{what will the visualization all the reader to do well} to \textit{how will the reader change.}  Statement not intended to be weirdly meta... intended to convey the specific idea that the we want cognitive and affective changes in the reader.

Blooms is Cool~\cite{anderson2001taxonomy}



Journalism - don't actually want neutrality. Cognitive change in state of the recipient is key.

Expressiveness -- 

Visualization can't be treated in isolation.  Either consider the insight offered implicitly or explicitly. Or the visualization serves as scaffolding for other learning objectives.  E.g. in order for you to understand X, you need to understand Y.

Take visualization of letter distributions in the English language. Letter 'E' is most popular, and appears 12.7\% of time in English. This 'fact' can be: (1) reinforced by vis (dual coding), (2) 'proven' by vis, (3) Increase salience and thereby increase recall, (4) fact is actually representative of a class of other related facts that I want you to pull. I'm suggesting: (a) how to read the diagram, and (b) what an interesting fact looks like.

\url{https://en.wikipedia.org/wiki/Letter_frequency}

But why do we need the other letter? Convention or it serves some other purpose.




Recall as metric, not totally compelling and certainly doesn't cover everything and narrative -- strategy, not an objective. Persuasion (rhetorical argument) -- but persuade to what end?

Annotation techniques --> pull to make things more salient

Wikipedia commons criteria: ``Must be realistically useful for an educational purpose'' (\url{https://commons.wikimedia.org/wiki/Commons:Project_scope})

The communicative visualization represents a partial trace/view of the analyst's process. It captures the internal set of logics by which either the analyst arrived at their conclusion or by which they think will act as evidence for the reader (based on the model of the analyst). Compresses the hypothesis - proof (Galileo example in Tufte, pg 108)

Reader as micro-analyst. The reader experiences a constrained environment, one set out not by the evidence of the data but interpreted/mediated by a set of humans. The first goal of which is ``believe me'' the second of which is some other cognitive change... remember me, make better decisions using me, etc.

Visual communication provides evidence -- is belief inherently a learning objective? Or is it simply an intermediate thing? a tactic? much like storytelling.

"student should believe" -- is this a reasonable LO? Even if it is, it is still testable. If it is not... if it is something that is intermediate... we can ask: does belief help in the specific cognitive change.  

`` But if you don’t present your data to readers so they can see it, read it, explore it, and analyze it, why would they trust you?'' -- Cairo, Functional Art

``This process of evidence construction and representation, though not a black box but certainly a gray area, consists of all the decisions that \textit{cause} the published findings of a report. These decisions are made, to varying degrees, both in the spirit of doing analytical detective work to discover what is going on \textit{and} in the spirit of advancing a favored point of view.'' -Tufte


Anti-LOs... those things that we do NOT want the reader to learn. APT (expressiveness)

Same visualization changes in task based on context -- among other visualizations in the hands of the analyst 


Most people when they hear about learning think back to their childhoold type. Passive does not mean without opinion or agency. Difference between pedagogy (structured and formal) and andragogy (aka adult or lifelong learning).

Knowles: ``Need to know: Adults need to know the reason for learning something.
Foundation: Experience (including error) provides the basis for learning activities.
Self-concept: Adults need to be responsible for their decisions on education; involvement in the planning and evaluation of their instruction.
Readiness: Adults are most interested in learning subjects having immediate relevance to their work and/or personal lives.
Orientation: Adult learning is problem-centered rather than content-oriented.
Motivation: Adults respond better to internal versus external motivators.''  Andragogy is still not well theorized. Pedgagogy has received significantly more attention.

\textit{entering behaviors} $=$ inputs

Different kinds of learning objectives. Modes of communicative vis... Active and post. Objective while reading, objective after. Layering by background of reader, how surprising the result. 




If we build it, they will come.. Karpiejev and Roth if we show the data properly the user will believe it. The user will believe the facts if we make sure they are evident in the plot. (APTish)~\cite{Kerpedjiev:2000:MCG:325737.325814}. The whole automated community is focused on making sure the fidelity of the message is high but not in ensuring that the goal of the creator is preserved. It's hard to model that. Making sure translation works.


Passive analyst versus active analyst. -- Active analyst creates visualization to guide the passive analyst. The passive analyst is the student/viewer. Active analyst mentors the passive.


Usually we ask questions about the vis as you see it. Los also ask what happens when you take the vis away.

Make vis viral/transmittable. You should be able to explain.

``A set of facts is expressible in a language if it contains a sentence that
(1) encodes all the facts in the set,
(2) encodes only the facts in the set.''~\cite{mackinlay1986automating}


Communicative function --> but how do we evaluate whether we've been successful at "communicating." Example: two ways of showing the data, both communicate/express the same facts, but how do I pick one over the other. Task language of communication is simply not sufficient. The ability to decode not enough. Argument for: existing task languages are not sufficient.

Our goal is explicitlely to assess the teacher, not the student.




The "while reading" test. If the vis doesn't support the LO at the time of reading, it likely won't support it after.



Designers have a vague notion that they are teaching. They often describe the goal of having their reader or audience `understand' something. Unfortunately, `understand' is a vague cognitive process. One that is generally frowned upon in the definition of learning objectives since we don't know what cognitive process understand refers to and consequently can't evaluate it.



\subsection{Alternative Learning Objective Taxonomies}
A complete discussion of alternative learning objective taxonomies is beyond the scope of this paper. We briefly describe alternative frameworks that we ultimately rejected.

A popular alternative to Bloom is the Structure of Observed Learning Outcomes (SOLO) framework. With SOLO, instructors often ask a ``what did you learn?'' and use a rubric for describing a student's achievement. The appeal of the framework as put by the author of SOLO, ``The difference, essentially, is that the Bloom levels are \textit{a priori} ones, imposed in advance by the teacher; whereas we would prefer to use levels that arise `naturally' in the understanding of the material''~\cite{biggs2014evaluating}. However, what is a bug for SOLO is a feature for us. We want communicative visualization to be \textit{designed}. \textit{A priori} formulation of objectives is critical to control the process. Understanding by Design (UbD)~\cite{wiggins2005understanding} is an alternative framework. UbD offers six facets: can explain, can interpret, can apply, has perspective, can empathize, has self-knowledge. These facets are not inherently structured and combine cognitive and affective objectives. The lack of structure may make it easier to construct objectives, but harder to evaluate them.

Finally, the DIKW taxonomy~\cite{dikw,zins07}--Data, Information, Knowledge, and Wisdom--is not principally a learning science innovation. DIKW features is often depicted in a hierarchical structure where `learning' at each level is needed for the next (data becomes information becomes knowledge becomes wisdom). However, the hierarchy has little to say about the specific cognitive processes that transform one to the next or explain how the elements are used (the `verbs'). 
This participant also noted that some ways of thinking  different fields ---journalism, data science, user experience, etc.--- and these fields all have different, although sometimes similar, ways of thinking about the reader/audience/user and the designer (or user's) goal for the visualization. Explicit thinking about intent or goals for what you want your viewer to achieve can be helpful in the design process. 
